A Deep Dive into NFT Whales: A Longitudinal Study of the NFT Trading Ecosystem

NFT (Non-fungible Token) has drastically increased in its size, accounting for over \$16.9B of total market capitalization. Despite the rapid growth of NFTs, this market has not been examined thoroughly from a financial perspective. In this paper, we conduct methodical analyses to identify NFT market movers who play a significant role in potentially manipulating and oscillating NFT values. We collect over 3.8M NFT transaction data from the Ethereum Blockchain from January 2021 to February 2022 to extract trading information in line with the NFT lifecycle: (i) mint, (ii) transfer/sale, and (iii) burn. Based on the size of held NFT values, we classify NFT traders into three groups (whales, dolphins, and minnows). In total, we analyze 430K traders from 91 different NFT collection sources. We find that the top 0.1\% of NFT traders (i.e., whales) drive the NFT market with consistent, high returns. We then identify and characterize the NFT whales' unique investment strategies (e.g., mint/sale patterns, wash trading) to empirically understand the whales in the NFT market for the first time.

==> sections/outdated/impact_old.tex <==
To examine how influential whales are in NFT ecosystem, we analyze whales' trading behavior in terms of their impact on the market sentiment and traders.

\subsection{Whales' Impact on NFT Market}
In this section, we analyze whales' transaction patterns in comparison with other groups. We study their effect on NFT ecosystem along with the evolution of NFT market.
%전반적으로 whale, dolphin, minnow 순으로 buy, recv, mint 많이  / sell, send 적게
%시장의 크기는 12월 점점 커지는데, 유저수에 비해 거래량은 많지 않음.
% Since whale's behavior greatly affects the flow of the market, it is essential to study how they trade across the evolution of NFT ecosystem. 
Figure \ref{f:long_tx} shows the monthly number of each transaction type of each group on average. We consider \textit{token\_count} in transaction data as one transaction. As mentioned in section 3.2., transaction types include \textit{buy, sell, receive, send, mint}, and \textit{burn}. 

Overall the average number of transactions by whales is overwhelmingly large. 
Note that y axis of each graph in Figure \ref{f:long_tx} has different scale. 
% Their activity seems to be decrease a lot in the second half, however, in the case of whale, transactions between traders have decreased and transfers through contract addresses have increased (Figure ? in the Appendix). 
Particularly noteworthy is the fact that trading activities of dolphins and minnows tend to be similar, while whales show much more fluctuations. To understand whales' behavior, we study how they respond to real-world events related to NFT. 

\noindent{\bf Sale (Buy/Sell).}
Whale group's buying pattern is similar to other groups, but their selling pattern is different. 
%돌고래, 민노우는 비슷한 패턴
%고래는 buy는 비슷, sell은 달라
This indicates that they buy tokens according to the market trend, but they only sell them with their own standards. 
Their behavior pattern over time is explained with several events (E1$\sim$E3) that whales had a huge impact on the market.
First, we observe a rapid but short-lived peak in February 2021 in all groups. With the growing popularity of \textit{Hashmasks}\cite{hashmasks}, traders buy a huge number of tokens of the collection, which accounts for more than half of their purchases.

\textbf{(E1)} However, in April, NFT market conditions cooled abruptly. Traders in all groups barely participated in transactions, because of the sharp decline (nearly 70\%) in the average price of NFTs \cite{NFT_burst}. In fact, before the market crash, whales' activities drop to the lowest position first, in March. This implies that decrease in whale's activities have had a big impact on the NFT market sentiment.
% price and flow of the NFT ecosystem.
\textbf{(E2)} In May, there exists an uplift in number of sells only in the whales' transaction graph. They sell tokens they minted on this month. The interesting fact is that 95\% of these tokens are from two new collections, \textit{Meebits} and \textit{Bored Ape Yacht Club (BAYC)}. 
\textit{Meebits} received the spotlight even before the launch, since it is made by the creators behind \textit{CryptoPunks}. 
On the other hand, \textit{BAYC} suddenly gained popularity due to a large quantity of whales' mint \cite{bayc_boom}. This promoted the sales of BAYC tokens, especially in dolphin and minnow group. In fact, \textit{BAYC} accounts for 40\% and 54\% of dolphins' and minnows' sales, respectively. 
% The interesting fact is that one of whales, who minted \textit{BAYC} the most (around 1K) and even advertised his minting on Twitter, sold almost all of the tokens to dolphins and minnows by June.
\textbf{(E3)} Overall sales volume ramps up steadily by July 2021, and increases dramatically in August. This is related to a surge in price of \textit{CryptoPunks} by whales. One day in August, a whale bought over 100 \textit{CryptoPunks} NFTs worth more than \$6M in total. Not long after, some of other whales bought tokens of this collection for \$3.7M and \$5.4M. Since then, whales' purchase of the collection continued. Whales' activities led to public interest in NFT market and new traders drastically swelled \cite{CryptoPunk_resurge}.
% an increased trading volume due to growing interest in \textit{Art Blocks} according to Google Trend.

In December, as famous fashion brands (e.g., such as Adidas and Nike) formed NFT partnerships or acquired NFT startups\cite{fashion_nft}, NFT gained greater attention from the public, which made a small increase in three groups. 

To sum up, it turns out three events (E1 $\sim$ E3) out of five were caused by whales, which verifies a great impact of whales in the NFT market.

\noindent{\bf Transfer (Receive/Send).}
%receive를 거의 다, send는 거의 앙ㄴ 함
In the beginning, whales barely do transfer, but from August, the number of transfer becomes greater than or equal to the number of sale. However, for the entire period of our data, among transfer types, whale rarely send NFTs but only receive them. 
%From September, most of the received tokens are related to game, which is consistent with the surge in popularity of decentralized NFT games at that time. 
This is in stark contrast to the fact that dolphins and minnows participate in sale much more than transfer. This represents dolphins increase their holding value through buying tokens, while whales increase by receive them during the second half. 
Interestingly, when we observe whales who receive NFTs a lot, they have a few main senders, and they get hundreds of tokens in a specific collection from each sender.
% When we observe traders who receive NFTs a lot, almost all of them have their own a few main senders, which is completely contrast to buy. This implies that some traders have a close relationship through transfer. 

\noindent{\bf Mint and Burn.}
% Unlike \textit{Meebits}, \textit{Bored Ape Yacht Club} did not gain much attention at the beginning of their launch. However, as soon as several whales minted a large number of \textit{BAYC} tokens, the rest of the tokens were all minted within a few hours\cite{bayc_boom}. This event also verifies the influence of whales on the market. 
We observe all three groups actively participate in mint, especially whale group. By September, mint is the most common transaction type of whales, meaning that they increase their holding value not only through buy, but also through mint.
There are three conspicuous points in their mint. 
In January 2021, they mint about four times more than any other transaction types, and most of them are \textit{Hashmasks}. It surged again in May, due to \textit{Meebits} and \textit{BAYC} as mentioned above. 
In later months including August, some collections(e.g.,\textit{Punks Comic} and \textit{MetaHero Universe: Planet Tokens}) embed governance rights on tokens(a.k.a. DAO tokens), that rose the demand for mint. For example, traders received \textit{Punks Comic} DAO tokens by burning their previous tokens of the collection.
This suggests that whales are interested in exercising governance rights on a collection. 
Noteworthy is whales only mint a huge amount of specific collections, while other groups mint various collections. Besides, we find and explain several unique characteristics of whales' mint in Section 5.3.

NFT market capitalization is increasing due to rise in the number of collections and traders. However, traders' practical activities rather decreased compared to early months. In fact, the number of active minnows is only 20\% of minnow group as of February 2022 (in Table \ref{t:active_users} of Appendix). This implies that NFT market is mainly operated by whale and dolphin group. In addition, we cannot observe any noticeable increase in whales' transactions after August, which means that no more influential collections emerged (e.g., \textit{CryptoPunks}). Despite the large number of collections' launch, a few major collections account for the majority of NFT market capitalization \cite{?}. Hence, holding NFTs of major collections can let whales keep their place.\\
%8월 이후에는 눈에 띄게 큰 변화가 없다. 그 뜻은 cryptopunks, bayc처럼 큰 콜렉션이 등장하지 않았다는 뜻. > 실제로 봤더니 엄청나게 많은 콜렉션이 등장했음에도 불구하고, 전체 시장 가치의 ?퍼센트를 얘네가 차지하더라. 결국 원래 고래였던 애들이 그 콜렉션을 계속 들고 있으면 계속 고래. 

\noindent{\bf Findings and Insight.}
NFT market is predominantly being driven by whales. They take various behaviors in the right place, resulting in their trading pattern being very distinct from other groups. Moreover, they have a huge impact on the market and often alter market sentiment.

% Specifically, the main focus of whales is {\it mint}, {\it } and whales commonly cherry pick high profile NFT collections and participate in the minting process of those collections.  

\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/sale_w.pdf}
         \caption{Sale graph}
         \label{f:sale_graph}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering         \includegraphics[width=\textwidth]{figures/trans_w.pdf}
         \caption{Transfer graph}
         \label{f:trans_graph}
     \end{subfigure}
        \caption{Trading network including whales from January 2022 to February 2022. Red, purple and green each represents whale, dolphin, and minnow. The size of the node is proportional to its PageRank.}
        \label{f:transaction_graph}
\end{figure}


% size가 작은 그룹일수록 holding leader가 많음, transfer 비율이 높음 
\subsection{Whales' Importance in Trading Network}
In this section, we explore the influence of whales on other traders by looking at the \textit{trading network}. \textit{Trading network} is a network formed by transactions between traders. Each node represents a trader, and edge represents transaction (sale or transfer) between them. The direction of the edge represents the transaction flow from sender to receiver.
% Dark-blue, sky-blue and olive each represent whale, dolphin, and minnow and the node size is proportional to its pagerank.
Since the structure of trading network gradually becomes apparent over time, Figure \ref{f:transaction_graph} only shows transactions from January 2022 to February 2022. Each graph shows trading network formed either by sale or transfer. To understand relationships between whale and the others, we only use transactions including whales for analysis. Whales' importance in the trading network is represented by PageRank \cite{brin1998anatomy}, generally used in web network graphs. 

The major finding is that whales show different relationships with traders in sale and transfer.
% 
That is, (1) The transfer network shows many noticeably large whales with high PageRank, unlike the sale network. This indicates that whales play a more important role in the transfer netwoTo examine how influential whales are in NFT ecosystem, we analyze whales' trading behavior in terms of their impact on the market sentiment and traders.

\subsection{Whales' Impact on NFT Market}
In this section, we analyze whales' transaction patterns in comparison with other groups. We study their effect on NFT ecosystem along with the evolution of NFT market.
%전반적으로 whale, dolphin, minnow 순으로 buy, recv, mint 많이  / sell, send 적게
%시장의 크기는 12월 점점 커지는데, 유저수에 비해 거래량은 많지 않음.
% Since whale's behavior greatly affects the flow of the market, it is essential to study how they trade across the evolution of NFT ecosystem. 
Figure \ref{f:long_tx} shows the monthly number of each transaction type of each group on average. We consider \textit{token\_count} in transaction data as one transaction. As mentioned in section 3.2., transaction types include \textit{buy, sell, receive, send, mint}, and \textit{burn}. 

Overall the average number of transactions by whales is overwhelmingly large. 
Note that y axis of each graph in Figure \ref{f:long_tx} has different scale. 
% Their activity seems to be decrease a lot in the second half, however, in the case of whale, transactions between traders have decreased and transfers through contract addresses have increased (Figure ? in the Appendix). 
Particularly noteworthy is the fact that trading activities of dolphins and minnows tend to be similar, while whales show much more fluctuations. To understand whales' behavior, we study how they respond to real-world events related to NFT. 

\noindent{\bf Sale (Buy/Sell).}
Whale group's buying pattern is similar to other groups, but their selling pattern is different. 
%돌고래, 민노우는 비슷한 패턴
%고래는 buy는 비슷, sell은 달라
This indicates that they buy tokens according to the market trend, but they only sell them with their own standards. 
Their behavior pattern over time is explained with several events (E1$\sim$E3) that whales had a huge impact on the market.
First, we observe a rapid but short-lived peak in February 2021 in all groups. With the growing popularity of \textit{Hashmasks}\cite{hashmasks}, traders buy a huge number of tokens of the collection, which accounts for more than half of their purchases.

\textbf{(E1)} However, in April, NFT market conditions cooled abruptly. Traders in all groups barely participated in transactions, because of the sharp decline (nearly 70\%) in the average price of NFTs \cite{NFT_burst}. In fact, before the market crash, whales' activities drop to the lowest position first, in March. This implies that decrease in whale's activities have had a big impact on the NFT market sentiment.
% price and flow of the NFT ecosystem.
\textbf{(E2)} In May, there exists an uplift in number of sells only in the whales' transaction graph. They sell tokens they minted on this month. The interesting fact is that 95\% of these tokens are from two new collections, \textit{Meebits} and \textit{Bored Ape Yacht Club (BAYC)}. 
\textit{Meebits} received the spotlight even before the launch, since it is made by the creators behind \textit{CryptoPunks}. 
On the other hand, \textit{BAYC} suddenly gained popularity due to a large quantity of whales' mint \cite{bayc_boom}. This promoted the sales of BAYC tokens, especially in dolphin and minnow group. In fact, \textit{BAYC} accounts for 40\% and 54\% of dolphins' and minnows' sales, respectively. 
% The interesting fact is that one of whales, who minted \textit{BAYC} the most (around 1K) and even advertised his minting on Twitter, sold almost all of the tokens to dolphins and minnows by June.
\textbf{(E3)} Overall sales volume ramps up steadily by July 2021, and increases dramatically in August. This is related to a surge in price of \textit{CryptoPunks} by whales. One day in August, a whale bought over 100 \textit{CryptoPunks} NFTs worth more than \$6M in total. Not long after, some of other whales bought tokens of this collection for \$3.7M and \$5.4M. Since then, whales' purchase of the collection continued. Whales' activities led to public interest in NFT market and new traders drastically swelled \cite{CryptoPunk_resurge}.
% an increased trading volume due to growing interest in \textit{Art Blocks} according to Google Trend.

In December, as famous fashion brands (e.g., such as Adidas and Nike) formed NFT partnerships or acquired NFT startups\cite{fashion_nft}, NFT gained greater attention from the public, which made a small increase in three groups. 

To sum up, it turns out three events (E1 $\sim$ E3) out of five were caused by whales, which verifies a great impact of whales in the NFT market.

\noindent{\bf Transfer (Receive/Send).}
%receive를 거의 다, send는 거의 앙ㄴ 함
In the beginning, whales barely do transfer, but from August, the number of transfer becomes greater than or equal to the number of sale. However, for the entire period of our data, among transfer types, whale rarely send NFTs but only receive them. 
%From September, most of the received tokens are related to game, which is consistent with the surge in popularity of decentralized NFT games at that time. 
This is in stark contrast to the fact that dolphins and minnows participate in sale much more than transfer. This represents dolphins increase their holding value through buying tokens, while whales increase by receive them during the second half. 
Interestingly, when we observe whales who receive NFTs a lot, they have a few main senders, and they get hundreds of tokens in a specific collection from each sender.
% When we observe traders who receive NFTs a lot, almost all of them have their own a few main senders, which is completely contrast to buy. This implies that some traders have a close relationship through transfer. 

\noindent{\bf Mint and Burn.}
% Unlike \textit{Meebits}, \textit{Bored Ape Yacht Club} did not gain much attention at the beginning of their launch. However, as soon as several whales minted a large number of \textit{BAYC} tokens, the rest of the tokens were all minted within a few hours\cite{bayc_boom}. This event also verifies the influence of whales on the market. 
We observe all three groups actively participate in mint, especially whale group. By September, mint is the most common transaction type of whales, meaning that they increase their holding value not only through buy, but also through mint.
There are three conspicuous points in their mint. 
In January 2021, they mint about four times more than any other transaction types, and most of them are \textit{Hashmasks}. It surged again in May, due to \textit{Meebits} and \textit{BAYC} as mentioned above. 
In later months including August, some collections(e.g.,\textit{Punks Comic} and \textit{MetaHero Universe: Planet Tokens}) embed governance rights on tokens(a.k.a. DAO tokens), that rose the demand for mint. For example, traders received \textit{Punks Comic} DAO tokens by burning their previous tokens of the collection.
This suggests that whales are interested in exercising governance rights on a collection. 
Noteworthy is whales only mint a huge amount of specific collections, while other groups mint various collections. Besides, we find and explain several unique characteristics of whales' mint in Section 5.3.

NFT market capitalization is increasing due to rise in the number of collections and traders. However, traders' practical activities rather decreased compared to early months. In fact, the number of active minnows is only 20\% of minnow group as of February 2022 (in Table \ref{t:active_users} of Appendix). This implies that NFT market is mainly operated by whale and dolphin group. In addition, we cannot observe any noticeable increase in whales' transactions after August, which means that no more influential collections emerged (e.g., \textit{CryptoPunks}). Despite the large number of collections' launch, a few major collections account for the majority of NFT market capitalization \cite{?}. Hence, holding NFTs of major collections can let whales keep their place.\\
%8월 이후에는 눈에 띄게 큰 변화가 없다. 그 뜻은 cryptopunks, bayc처럼 큰 콜렉션이 등장하지 않았다는 뜻. > 실제로 봤더니 엄청나게 많은 콜렉션이 등장했음에도 불구하고, 전체 시장 가치의 ?퍼센트를 얘네가 차지하더라. 결국 원래 고래였던 애들이 그 콜렉션을 계속 들고 있으면 계속 고래. 

\noindent{\bf Findings and Insight.}
NFT market is predominantly being driven by whales. They take various behaviors in the right place, resulting in their trading pattern being very distinct from other groups. Moreover, they have a huge impact on the market and often alter market sentiment.

% Specifically, the main focus of whales is {\it mint}, {\it } and whales commonly cherry pick high profile NFT collections and participate in the minting process of those collections.  

\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/sale_w.pdf}
         \caption{Sale graph}
         \label{f:sale_graph}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering         \includegraphics[width=\textwidth]{figures/trans_w.pdf}
         \caption{Transfer graph}
         \label{f:trans_graph}
     \end{subfigure}
        \caption{Trading network including whales from January 2022 to February 2022. Red, purple and green each represents whale, dolphin, and minnow. The size of the node is proportional to its PageRank.}
        \label{f:transaction_graph}
\end{figure}


% size가 작은 그룹일수록 holding leader가 많음, transfer 비율이 높음 
\subsection{Whales' Importance in Trading Network}
In this section, we explore the influence of whales on other traders by looking at the \textit{trading network}. \textit{Trading network} is a network formed by transactions between traders. Each node represents a trader, and edge represents transaction (sale or transfer) between them. The direction of the edge represents the transaction flow from sender to receiver.
% Dark-blue, sky-blue and olive each represent whale, dolphin, and minnow and the node size is proportional to its pagerank.
Since the structure of trading network gradually becomes apparent over time, Figure \ref{f:transaction_graph} only shows transactions from January 2022 to February 2022. Each graph shows trading network formed either by sale or transfer. To understand relationships between whale and the others, we only use transactions including whales for analysis. Whales' importance in the trading network is represented by PageRank \cite{brin1998anatomy}, generally used in web network graphs. 

The major finding is that whales show different relationships with traders in sale and transfer.
% 
That is, (1) The transfer network shows many noticeably large whales with high PageRank, unlike the sale network. This indicates that whales play a more important role in the transfer network than the sale network. 
% Also, whales who buy tokens a lot, also sell a lot, however, they do not send them again.
% (1) In Figure \ref{f:sale_graph}, we observe whales of various sizes exist, and large dolphins and minnows are also seen. However, in Figure \ref{f:trans_graph}, a few extremely large whales and large size of non-whale traders barely exist. This means that the effect of a small number of whales on other trader is greater in transfer graph than in sale graph.
(2) Almost all whales transfer only with dolphins and minnows surrounding them, but they sale with whales (or the others) regardless of cluster.
% This is due to the observation of a lot of distinct clusters of dolphins and minnows surrounding a whale in Figure \ref{f:trans_graph}, which indicates that transactions occur mainly within each cluster. This is different with whale's \textit{sale}, such clusters appear unclear. 
(3) In the transfer graph, there are a lot of small independent components (WCCs) that are not connected to the biggest component. This phenomenon is hard to see in sale graph.

Since transfer is a transaction without actual payment, we can assume that traders are likely to be in a specific relationship. In other words, whales appear to form a \textit{whale-centered clusters} through transfer.
% (The number of weakly connected components in the transfer network is around three times that in the sale network). 
\\ 
%  This suggests that communities become more solid over time. In section 5.1., in the second half, we find the majority of whales' transactions are \textit{transfer}, which indicates that they mainly trade within the community rather than with external traders.\\
% Previous works \cite{casale2021networks}\cite{nadini2021mapping} show that traders are clustered around NFT collections. However, we discover it is only true when traders are in transfer relationship, not in sale relationship.
% 0.0029 max
% Diameter: 11,  Avg Path length: 3.0963156367856106
% Diameter: 24, Avg Path length: 8.026665147315253


\noindent{\bf Findings and Insight.}
Whales form close relationships with small number of traders through \textit{transfer-major communities}, focusing on specific collections. Some of them participate in wash trading, raising NFT prices.


%t = 10 모든 멤버가 holding leader로 이루어진 그룹이 있는데, 8명이 CyberKongz를 125번 transfer
%t = 13 4명이 800번, 6명이 470번 meebits transfer --> meebits 가격 증가 
rk than the sale network. 
% Also, whales who buy tokens a lot, also sell a lot, however, they do not send them again.
% (1) In Figure \ref{f:sale_graph}, we observe whales of various sizes exist, and large dolphins and minnows are also seen. However, in Figure \ref{f:trans_graph}, a few extremely large whales and large size of non-whale traders barely exist. This means that the effect of a small number of whales on other trader is greater in transfer graph than in sale graph.
(2) Almost all whales transfer only with dolphins and minnows surrounding them, but they sale with whales (or the others) regardless of cluster.
% This is due to the observation of a lot of distinct clusters of dolphins and minnows surrounding a whale in Figure \ref{f:trans_graph}, which indicates that transactions occur mainly within each cluster. This is different with whale's \textit{sale}, such clusters appear unclear. 
(3) In the transfer graph, there are a lot of small independent components (WCCs) that are not connected to the biggest component. This phenomenon is hard to see in sale graph.

Since transfer is a transaction without actual payment, we can assume that traders are likely to be in a specific relationship. In other words, whales appear to form a \textit{whale-centered clusters} through transfer.
% (The number of weakly connected components in the transfer network is around three times that in the sale network). 
\\ 
%  This suggests that communities become more solid over time. In section 5.1., in the second half, we find the majority of whales' transactions are \textit{transfer}, which indicates that they mainly trade within the community rather than with external traders.\\
% Previous works \cite{casale2021networks}\cite{nadini2021mapping} show that traders are clustered around NFT collections. However, we discover it is only true when traders are in transfer relationship, not in sale relationship.
% 0.0029 max
% Diameter: 11,  Avg Path length: 3.0963156367856106
% Diameter: 24, Avg Path length: 8.026665147315253


\noindent{\bf Findings and Insight.}
Whales form close relationships with small number of traders through \textit{transfer-major communities}, focusing on specific collections. Some of them participate in wash trading, raising NFT prices.


%t = 10 모든 멤버가 holding leader로 이루어진 그룹이 있는데, 8명이 CyberKongz를 125번 transfer
%t = 13 4명이 800번, 6명이 470번 meebits transfer --> meebits 가격 증가 


==> sections/outdated/whale_basic_old.tex <==
NFT whales have compared to the other whales in markets such as stock. In this section, we characterize NFT whales by scrutinizing trading patterns of NFT collections and how they manage assets in terms of holding period and trading price. 

% In this section, we investigate the overall features of NFT whales that are distinct from whales of other markets(e.g., stock market). We then scrutinize their holdings in terms of collections and price. Finally, we analyze the changes in whale group's composition.

% \subsection{Understanding NFT Whale}
\subsection{Whales' NFT Portfolio Management}
%콜렉션마다, 콜렉션 내의 토큰마다 완전 다른 가격 분포
% We take a close look at NFT whales in terms of the number of NFTs they have. First, we examine characteristics of 1) whale group and 2) whale individual in separate.
We describe how NFT whales manage their NFT portfolio in terms of token types, the number of holdings, collection preferences, and price distribution.

% \noindent{\bf Whale Group.}
\noindent{\bf The number of collections in portfolio.}
We investigate how many NFTs and how much NFT holding value whales have in the market.
As mentioned in Section 3, there are two types of tokens, ERC-1155 and ERC-721. Due to different interest of whale group on each token type, the quantity and holding value vary over time. 
In case of ERC-1155 tokens, until June 2021, the number of tokens held by whales is close to 0\% of the total tokens, which shows that whales were not interested in ERC-1155 tokens. However, from July, the quantity and holding value of their ERC-1155 tokens began to increase and reached 9.4\% and 24.3\% in August. This is likely to be due to the launch of \textit{Punks Comic} collection, and this interest continues to the early 2022 with the emergence of other famous ERC-1155 collections. 
% In the case of ERC-1155 tokens, it is possible to exist multiple tokens with the same pair of (\textit{token\_contract}, \textit{token\_id}).
Meanwhile, whales steadily had interest on ERC-721 tokens. The total quantity and average price of ERC-721 tokens are 4.3 times and 8.4 times larger than those of ERC-1155 tokens, respectively (as of February 2022). Therefore, whales group's holding value of ERC-721 tokens takes majority portion of entire holding value. To sum these two types of tokens all together, while whale group only possesses less than 5\% of the total quantity of NFTs, the total holding value accounts for around 20\% of the NFT market cap. This indicates that they have high-value NFTs than the other groups. The percentage of the number and value of tokens held by whale group is summarized in Table \ref{f:whale_distribution} of Appendix. 


\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/whale_dist.pdf}
    \caption{Token Distribution of Whales in February, 2022}
    \label{f:whale_distribution}
\end{figure}

% \noindent{\bf Whale Individual.}
Then we scrutinize each individual in the whale group by looking at the distribution of whales according to tokens they have. In Figure \ref{f:whale_distribution}, more than half of whales have only ERC-721 tokens and 93\% have more ERC-721 tokens than ERC-1155 tokens. Token quantity of whales ranges from 1 to 6,516, and the holding value ranges from \$1.2M to \$31.3M. Even within the whale group, the number and holding value of each whale's NFTs are very different. Interestingly, a whale with the highest holding value (the darkest point in the graph) has only 20 NFTs, which confirms that the number of NFTs they have is not significantly related to their NFT holding value. \\

\noindent{\bf Findings and Insight.}
Among two types of NFTs, almost all of whales prefer ERC-721 tokens. In NFT market, having a large quantity of NFTs does not lead to large holding value. This implies that whales mainly focus on possessing distinctive and valuable NFTs.    


\begin{figure}[ht!]
  \centering
  \includegraphics[width=0.8\linewidth]{figures/holding_distribution.pdf}
  \caption{Price distribution of holding tokens among different groups. For ERC-1155 tokens, there does not exist any token in range R6.}
  \label{f:price_dist}
\end{figure}


% \subsection{Whales' Holdings}
\subsection{Whales' Portfolio Holdings}
Participants in NFT market pursue financial gains. Thus, it is necessary to examine holdings in portfolio. In this section, we examine whale's NFT holdings in portfolio, preferences, and dominance in NFT collections.

% In this section, we enquire into the NFTs that are in hands of whales. We examine whether whales indeed monopolize the most of high-price tokens. 

\noindent \textbf{Top collection holdings.} We begin by searching for top 10 collections that whales mostly hold. Majority of the collections in top 10 are popular collections with large trading volume. Whales' most holding collection is \textit{Art Blocks} where 9.6K tokens are held by whales. Interestingly, whales hold 1.6K \textit{CryptoPunks} tokens which accounts for 16\% of total tokens in this collection. Whales' holding token numbers for remaining collections can be found on Table \ref{t:whale_collections} of Appendix.

\begin{figure*}[t!]
  \centering
  \includegraphics[width=0.9\linewidth]{figures/sankey.pdf}
  \caption{Top : Changes in the group of traders in \textit{whale} at least once from January 2021 (t = 1) to August 2021 (t = 8), Bottom : Changes in the group of traders in \textit{whale} at least once until February 2022 (t = 14). (Dark-blue, sky-blue, olive, and grey in the graph each represents whales, dolphins, minnows, and traders who never traded before, and they are noted as from A to D. Transitions from one color to another depict a quantity of traders with group changes.) } 
  \label{f:sankey}
\end{figure*}


\noindent\textbf{Price distribution.} To look into price of each group's holdings, we divide the token price into a number of ranges, from \$0 to \$23.3M. Due to this large range, we divide each range with log scale. Figure \ref{f:price_dist} is the price distribution of tokens that each group holds on February 28, 2022. Figure \ref{f:price_dist}(a) and (b) each shows distribution of ERC-721 and ERC-1155 tokens on all 91 collections. On the other hand, \ref{f:price_dist}(c) shows token price within a collection, \textit{Cryptopunks}. Note that the price distribution of popular collections (e.g., \textit{BAYC, Art Blocks}) also resembles the distribution of \textit{Cryptopunks}. Almost all of the tokens with price over \$10M are in hands of whales. In addition, whales are the most holders tokens in range \$1M to \$10M across all collections and within a collection. All three of the graphs in Figure \ref{f:price_dist} reveal whales are the only holders of the high-price tokens.\\



\noindent\textbf{Findings and Insight.} 
Generally speaking, price of a good in a market is an indicator of the `value'. The result of this section suggests that whales gain dominance over almost all of highly valuable tokens.




\subsection{Changes in Whales' Composition}

NFT market changed dramatically during 14 months with the influx of new traders and the advent of various types of new collections. In this rapidly changing market, how do traders become the whale group?
%In this highly volatile NFT market, has there been any change in whale composition?
To answer this question, we study how traders move between groups during 14 months, focused on whales. 
% We understand characteristics of whales according to the group they belonged to before, in terms of how they become whales.
%nft market은 새로운 nft도 많이 등장하고, 굉장히 급변하고 있는 시기인데, 그럼에도 불구하고 whale 대부분 남아있음
%whale 사이즈가 커지면서 돌핀이 남은 자리를 차지하는 건 당연.
%minnow에서 오는 비율 굉장히 적음.
%whale에서 non-whale되는 trader들의 절반 이상의 토큰이 send를 통해 new traders한테 감. -> 원래 whale과 specific relationship
%from minnows --> 대부분 recv 거의 없고, buy 혹은 mint --> 다른 유저와의 관계 x

Figure \ref{f:sankey} shows the changes in composition of whale group until February 2022. To better visualize the changes in the first half of the period, the top graph in Figure \ref{f:sankey} only covers traders who were in whale group at least once until August 2021. This is because the number of traders in February 2022 is around 70 times higher than that of January 2021.
The range of \textit{t} is from 1 to 14, indicating each month from January 2021 to February 2022.


In the beginning, since the size of whale group is small, the composition of the group is highly volatile as the market size increases. However, from June 2021 (t = 6), more than 80\% of whales remain in the next whale group, except for August 2021 (t = 8). From July to August, there is the biggest change in the composition of whale group. This is due to the fact that August 2021 is when the number of new traders appeared the most compared to the previous months, with the surge of public interest in NFT [?]. 
To understand how traders become whale group and how whales keep their status, we investigate the characteristics according to whale's origin as follows.

\noindent{\textbf{Whales from \textit{whale}.}}
They maintain their status through various ways: buy, receive, and mint. In the first half, more than half of whales use buy as their major way to increase holding value. However, in early 2022, whales who mainly receive tokens grow in number. Meanwhile, some actively mint NFTs. For example, a whale minted tremendous number of tokens in several collections and sold them to dolphins and minnows. There also exist traders who have not been active for more than a few months. Their extremely expensive tokens let them stay in whale group. \\
% These whales can be considered as \textit{whale} in specific collection, as well as in NFT ecosystem.\\  
% In this regards, information is important in \textit{mint} because it is often done at a specific time or may require certain conditions. As time goes by, most of the traders who participate in mint are belong to whale, which can be interpreted as sharing information among themselves. Therefore, it might be difficult to obtain information for mint if traders are not in whale. We will discuss about whale's mint in section 5.3.
\noindent{\textbf{Whales from \textit{dolphin}.}}
As the size of the whale group increases, it is natural for dolphins to become whales. In August, when the market size grow most rapidly, dolphins take up 39\% of new whale group. 
They raise their holding value in various ways like whales from \textit{whale}. However, in early 2022, new whales from dolphin reduce to 15\%.

% A special case is one from dolphin in August who minted about 1,000 \textit{Punks Comics} tokens, which is Pixel Vault account, the company behind the collection.

\noindent{\textbf{Whales from \textit{minnow}.}}
We rarely observe whales who formerly belonged to \textit{minnow}, usually none. 
They overall increase their NFT holding value through buy or mint. They barely receive tokens from other traders, which indicates that they do not have traders in a particular relationship. This is completely different to whales from traders who have never traded before described below.   


\begin{figure*}[ht]
  \centering
  \includegraphics[width=0.9\linewidth]{figures/long_tx_cnt.pdf}
  \caption{The average number of transactions involving \textit{Whale/Dolphin/Minnow} classes over time }
  \label{f:long_tx}
\end{figure*}

\noindent{\textbf{Whales from traders who have never traded before.}}
There are a lot of traders who became whales as soon as they participate in the NFT market. When the size of the market increases rapidly, whales from this group sometimes outnumber whales from dolphin group. They usually become whales through buy or receive, but many of them become whales only through receive.
Usually, the tokens they receive are NFTs of popular collections with high trading volume (e.g. \textit{CrytoPunks} and \textit{Art Blocks}). Interestingly, most of tokens they received come from traders who were whales at $t-1$ but are not at $t$.
This implies that they have a close tie with the former whales.\\ 
%9월 민트 많이해서 올라온 앧르 있음
\noindent{\bf Findings and Insight.}
Although the NFT ecosystem is rapidly growing, whales keep their place firmly. In addition, newly emerging whales are often associated with former whales. This clearly shows that it is hard for minnows to be whales, and thus to be a whale, one should strive to act out of the group.

% Overall the high ranks of traders who buy or receive a lot rarely overlap. When we observe traders who receive NFTs a lot in each group, almost all of them have their own a few main senders, which is completely contrast to buy. This implies that some traders have a close relationship through transfer, especially whales from D. We will discuss about relationship between whales and other traders in section 5.2. 
% We find out that it is very difficult for a trader to have a high holding value, other than buying  high value tokens or receiving tokens from previous whales in certain relationships. 
% , by investigating how they became whales depending on where they came from.



==> sections/tendency.tex <==
\subsection{Most-Valuable tokens}

